Guiding Through Complexity: What Makes Good Supervision for Hard Math Reasoning Tasks?

How can "weak teacher models" such as average human annotators or existing AI systems, effectively supervise LLMs to improve performance on hard reasoning tasks, especially those that challenge and requires expertise or daily practice from the teacher models? In this paper, we seek for empirical answers to this question by investigating various data-driven strategies that offer supervision data at different quality levels upon tasks of varying complexity. Two intuitive strategies emerge for teacher models to provide supervision during alignment training: 1) using lower-quality supervision from complete tasks that match the difficulty of the target reasoning tasks, and 2) leveraging higher-quality supervision from easier subtasks that are less challenging. Interestingly, we find that even when the outcome error rate for hard task supervision is high (e.g., 90\%), training on such data can outperform perfectly correct supervision of easier subtasks on multiple hard math benchmarks. We further identify a more critical factor influencing training performance: step-wise error rates, which indicate the severity of errors in solutions. Specifically, training on hard task supervision with the same outcome error rates but disparate step-wise error rates can lead to a 30\% accuracy gap on MATH benchmark. Our results also reveal that supplementing hard task supervision with the corresponding subtask supervision can yield notable performance improvements than simply combining rephrased hard full task supervision, suggesting new avenues for data augmentation. Data and code are released at https://github.com/hexuan21/Weak-to-Strong.

==> tables/3.2_full_sub_eg.tex <==
% \begin{table}[h]
%     \centering
%     \begin{subtable}[t]{0.32\textwidth} 
%         \centering
%         \begin{tabular}{p{0.9\textwidth}}
%             \toprule
%             \textbf{Hard task (full task)}\\
%             Find the range of real numbers $m$ for which the quadratic equation $x^2 + (m-1)x + 1 = 0$ has solutions in the interval $[0,2]$\\
%             \midrule
%             \textbf{Solution}\\
%             \bottomrule
%         \end{tabular}
%         \caption{First subtable}
%     \end{subtable}
%     \hspace{0.1cm} 
%     \begin{subtable}[t]{0.32\textwidth} 
%         \centering
%         \begin{tabular}{p{0.9\textwidth}}
%             \toprule
%             \textbf{Easy task 1 (sub-task 1)}\\
%             Determine the values of $ m $ for which the discriminant of the quadratic equation $ x^2 + (m-1)x + 1 = 0 $ is non-negative. \\
%             \midrule
%             \textbf{Solution}\\
%             \bottomrule
%         \end{tabular}
%         \caption{Second subtable}
%     \end{subtable}
%     \hspace{0.1cm} 
%     \begin{subtable}[t]{0.32\textwidth} 
%         \centering
%         \begin{tabular}{p{0.9\textwidth}}
%             \toprule
%             \textbf{Easy task 2 (sub-task 2)}\\
%             Find the values of $ m $ such that the value of $ x^2 + (m-1)x + 1 = 0 $ evaluated at $ x = 2 $ is non-negative.\\
%             \midrule
%             \textbf{Solution}\\
%             \bottomrule
%         \end{tabular}
%         \caption{Third subtable}
%     \end{subtable}
%     \caption{Main table caption}
% \end{table}











\begin{table*}[t]
\vspace{-2.5em}
\renewcommand{\arraystretch}{1.2}
\small
\centering
\scalebox{0.8}{
\begin{tabular}{p{1.2\textwidth}}
\toprule

\textbf{Hard Full Task} \\
Find the range of real numbers $m$ for which the quadratic equation $x^2 + (m-1)x + 1 = 0$ has solutions in the interval $[0,2]$\\

\textbf{Solution} \\
For the quadratic equation $x^2 + (m-1)x + 1 = 0$ to have solutions in the interval $[0,2]$, it must satisfy certain conditions related to its discriminant and the values of $x$ at the endpoints of the interval.\\

First, let's consider the discriminant of the equation, $\Delta = (m-1)^2 - 4*1*1 = m^2 - 2m - 3$. For the equation to have real solutions, the discriminant must be non-negative, $\Delta \geq 0$. This gives us $m^2 - 2m - 3 \geq 0$, which simplifies to $(m-3)(m+1) \geq 0$. This inequality holds for $m \leq -1$ or $m \geq 3$.\\

However, we also need to ensure that the solutions are within the interval $[0,2]$. By evaluating the quadratic equation at the endpoints of the interval, we get:\\

1. For $x=0$: $0^2 + (m-1)0 + 1 = 1$, which is always positive.\\
2. For $x=2$: $2^2 + (m-1)2 + 1 = 4 + 2m - 2 + 1 = 2m + 3$, which needs to be non-negative for the solutions to lie within the interval. This gives us $2m + 3 \geq 0$, simplifying to $m \geq -\frac{3}{2}$.\\

Combining these conditions, we find that the range of $m$ for which the quadratic equation has solutions in the interval $[0,2]$ is $\boxed{(-\infty, -1)}$.\\
\midrule

\textbf{Easy Subtask 1} \\
Determine the values of $ m $ for which the discriminant of the quadratic equation $ x^2 + (m-1)x + 1 = 0 $ is non-negative. \\
\midrule

\textbf{Easy Subtask 2} \\
Find the values of $ m $ such that the value of the quadratic equation $ x^2 + (m-1)x + 1 = 0 $ evaluated at $ x = 2 $ is non-negative.\\

\bottomrule
\end{tabular}
}
\caption{Example to showcase the task decomposition for obtaining easy subtasks.}
% \vspace{-6pt}
\label{tab:3.2_full_sub_eg}
\end{table*}

==> tables/_discard_7_combine_2epoch_rephrase.tex <==
\begin{table*}[t]
    \centering
    \vspace{-3.5em}
    \begin{subtable}[ht]{0.48\textwidth}
    \centering
    \scriptsize
    \scalebox{0.82}{
    \begin{tabular}{lcccccc}
    \toprule
    \multirow{2}{*}{\textbf{Tasks}} & \multicolumn{2}{c}{\textbf{Combination 1}}                             & \multicolumn{2}{c}{\textbf{Combination 2}}                             & \multicolumn{2}{c}{\textbf{Combination 3}}                             \\
    \cmidrule(lr){2-3}
    \cmidrule(lr){4-5}
    \cmidrule(lr){6-7}
                           & (50\%, 10\%) & 50\% & (80\%, 40\%) & 80\% & (20\%, 10\%) & 20\% \\
    \midrule
    MATH           & \hlpink{48.6}                                    & 47.8               & \hlpink{43.8}                                    & 43.2               & \hlpink{48.0}                                    & 47.4               \\
    Olympic-Arena                       &  12.7                                       &  12.7                  &  \hlpink{14.1}                                       &  13.6                  &  12.7                                       &  12.7                  \\
    JEE-Bench                       &  \hlcyan{11.7}                                       &  12.3                  &  12.3                                       &  12.3                  &   \hlpink{8.0}                                      &  7.4                  \\
    Gaokao-Mathcloze                       &  \hlpink{45.8}                                       &  44.1                  &   \hlpink{42.4}                                      &  40.7                  &  39.0                                       &  39.0                  \\
    SAT-Math                       &  \hlpink{61.0}                                       &  60.0                  &   \hlpink{60.0}                                      &   58.2                 &  \hlpink{59.1}                                       &  58.2     \\ 
    \bottomrule
    \end{tabular}
    }
    \caption{Combined vs. Hard task supervision.}
    \vspace{-3pt}
    \label{tab:combination-analysis}
    \end{subtable}
    \hfill
    \begin{subtable}[ht]{0.48\textwidth}
    \centering
    \scriptsize
    \scalebox{0.82}{
    \begin{tabular}{lccc}
    \toprule
    \multirow{2}{*}{\textbf{Tasks}} & \multicolumn{3}{c}{\textbf{Combination}}                                     \\
    \cmidrule(lr){2-4}
                           & (50\%, 10\%) & 50\% (4 Epochs) & 50\% (Merge Rephrased.) \\
    \midrule
    MATH           & \hlpink{48.6}                                    & 45.0       &   48.4                \\
    Olympic-Arena                       &  12.7                                       &   12.7           &     12.7                   \\
    JEE-Bench                       &  \hlpink{11.7}                                       &  9.2         &   10.4                        \\
    Gaokao-Mathcloze                       &  \hlpink{45.8}                                       &  42.4            &   44.1                     \\
    SAT-Math                       &  \hlpink{61.0}                                       &  55.5          &  57.3          \\ 
    \bottomrule
    \end{tabular}
    }
    \caption{Combined vs. 4 Epochs vs. Merge Rephrased.}
    \vspace{-3pt}
    \label{tab:compare-with-double-epochs}
    \end{subtable}
% \caption{Accuracy (\%) of methods for enhancing performance beyond two epochs of hard task supervision: ``4 Epochs'' refers to the baseline, which involves training for twice the number of epochs. ``Merge Rephrased'' indicates the baseline where LLMs are trained using a combined dataset of the original hard task supervision and its rephrased versions.}
% ========= replaced by the paragraph below. 
\caption{Accuracy (\%) of methods for improving performance beyond two epochs of hard task supervision: "4 Epochs" refers to the baseline of training for double the epochs, while "Merge Rephrased" denotes training the data that combines the original hard tasks with the rephrased versions.}
\vspace{-9pt}
\label{tab:_discard_combination-and-other-baselines}
\end{table*}
